Quantifying Model Complexity via Functional Decomposition for Better Post-Hoc Interpretability

Post-hoc model-agnostic interpretation methods such as partial dependence plots can be employed to interpret complex machine learning models. While these interpretation methods can be applied regardless of model complexity, they can produce misleading and verbose results if the model is too complex, especially w.r.t. feature interactions. To quantify the complexity of arbitrary machine learning models, we propose model-agnostic complexity measures based on functional decomposition: number of features used, interaction strength and main effect complexity. We show that post-hoc interpretation of models that minimize the three measures is more reliable and compact. Furthermore, we demonstrate the application of these measures in a multi-objective optimization approach which simultaneously minimizes loss and complexity.

==> latex-math/chapter-notation.tex <==
\section{General Notation and Terminology}
\label{sec:notation}

Consider a $p-$dimensional feature space $\Xspace = (\Xspace[1] \times \Xspace[2] \times \hdots \times \Xspace[p])$ %of arbitrary measurement scales
and a target space $\Yspace$.
Suppose that there is an unknown functional relationship $f$ between $\Xspace$ and $\Yspace$.
ML algorithms try to learn this relationship using training data with observations that have been drawn i.i.d. from an unknown probability distribution $\mathcal{P}$ on the joint space $\Xspace \times \Yspace$.
%The learned prediction model will be denoted by $\fh$ and approximates $f$.
We consider an arbitrary prediction model $\fh$, fitted on some training data to approximate $f$ and analyze it with model-agnostic interpretability methods.
Let $\D = \Dset$ be a test data set sampled i.i.d. from $\mathcal{P}$ where $n$ is the number of observations in the test set.
Let $P = \{1, \hdots, p\}$ be an index set referring to all features.
We denote the corresponding random variables generated from the feature space by $X = (X_1, \hdots, X_p)$ and the random variable generated from the target space by $Y$.
In our notation, the vector $\xi = \xivec \in \Xspace$ refers to the $i$-th observation which is associated with the target outcome $\yi \in \Yspace$ and $\xj = \xjvec$ denotes the realizations of the $j$-th feature.
%Suppose that there is an unknown functional relationship $f$ that maps each observation $\xi$ to its target outcome $\yi$.
% Performane estimation
% The performance estimation of a ML algorithm is based on training the algorithm on training data and estimating the \emph{generalization error} (also known as \emph{test error}) of the algorithm on new (unseen) test data.
We denote the generalization error of a fitted model on unseen test data from $\mathcal{P}$ by $GE(\fh, \mathcal{P}) = \E(L(\fh(X), Y))$, measured by a loss function $L$.
%with which the performance of $\fhD$ is measured.
It can be estimated using the test data $\D$ by %through the empirical expected loss
%by splitting the observed data $\D$ into a training set $\Dtrain$ and test set $\Dtest = \D \setminus \Dtrain$, fitting the model on the training set and averaging the loss or gain function over an independent test set using
\begin{equation}
\label{eq:geest}
%\GEh{}(\fh, \D) = \frac{1}{|\D|} \sum_{\xy \in \D} L(\fh(x), y).
\textstyle \GEh{}(\fh, \D) = \frac 1 n \sum_{i=1}^n \Lii.
\end{equation}
%Note that if $\fh$ was trained on $\D$ and if the generalization error uses again $\D$ to measure the performance, we obtain an estimate for the training error.
%We therefore consider $\fh$ as a fixed model that was trained on $\Dtrain$ which is i.i.d. from $\D$. %the observations from the data set $\D$ were not used to fit the model $\fh$.
A better estimate for the generalization error of an ML algorithm can be obtained using resampling techniques such as cross-validation or bootstrap \citep{Bischl2012}. %as they %reuse the observed data at hand to produce a better estimator.
%Specifically, they repeatedly split the observed data into training and test sets of equal size, fit a model using the produced training sets and estimate the performance on the remaining test sets.
%The resulting performance values on each test set are then aggregated by averaging in order to estimate the generalization error more precisely \citep[see e.g.][]{Bischl2012}.


==> latex-math/ml-bagging.tex <==
% ml - bagging, random forest

\newcommand{\bl}[1]{b^{[#1]}(x)}											% baselearner with argument for m
\newcommand{\blm}{\bl{m}}												    % baselearner without argument for m
\newcommand{\blmh}{\hat{b}^{[m]}(x)}										% estimated base learner 
\newcommand{\fM}{f^{[M]}(x)}                    % ensembled predictor


==> latex-math/ml-boosting.tex <==
% ml - boosting
\newcommand{\fm}{f^{[m]}}                                                   % prediction in iteration m
\newcommand{\fmh}{\hat{f}^{[m]}}                                            % prediction in iteration m
\newcommand{\fmd}{f^{[m-1]}}                                                % prediction m-1
\newcommand{\fmdh}{\hat{f}^{[m-1]}}                                         % prediction m-1
\newcommand{\bmm}{b^{[m]}}                                                  % basemodel m
\newcommand{\bmmh}{\hat{b}^{[m]}}                                           % basemodel m with hat
\newcommand{\betam}{\beta^{[m]}}                                            % weight of basemodel m
\newcommand{\betamh}{\hat{\beta}^{[m]}}                                     % weight of basemodel m with hat
\newcommand{\betai}[1]{\beta^{[#1]}}                                        % weight of basemodel with argument for m
\newcommand{\errm}{\text{err}^{[m]}}                                        % weighted in-sample misclassification rate
\newcommand{\wm}{w^{[m]}}                                                   % weight vector of basemodel m
\newcommand{\wmi}{w^{[m](i)}}                                               % weight of obs i of basemodel m
\newcommand{\thetam}{\theta^{[m]}}                                          % parameters of basemodel m
\newcommand{\thetamh}{\hat{\theta}^{[m]}}                                   % parameters of basemodel m with hat
\newcommand{\rmm}{r^{[m]}}                                                  % pseudo residuals
\newcommand{\rmi}{r^{[m](i)}}                                               % pseudo residuals
\newcommand{\Rtm}{R_{t}^{[m]}}                                              % terminal-region
\newcommand{\Tm}{T^{[m]}}                                                   %
\newcommand{\ctm}{c_t^{[m]}}                                                % mean, terminal-regions
\newcommand{\ctmh}{\hat{c}_t^{[m]}}                                         % mean, terminal-regions with hat
\newcommand{\ctmt}{\tilde{c}_t^{[m]}}                                       % mean, terminal-regions
\newcommand{\fxk}{f_k(x)}                                                   % f_k(x)
\newcommand{\Lp}{L^\prime}
\newcommand{\Ldp}{L^{\prime\prime}}
\newcommand{\Lpleft}{\Lp_{\text{left}}}

==> latex-math/ml-mbo.tex <==
% ml - MBO
\newcommand{\sxh}{\hat{s}(x)} % uncertainty shat(x)
\newcommand{\vxh}{\hat{s}^2(x)}
\newcommand{\matK}{\mathbf{K}}
\newcommand{\kstarx}{\mathbf{k}_*(x)}
\newcommand{\xpi}[1][i]{x^{*(#1)}}
\newcommand{\vhx}{\ensuremath{\sh^2(\xv)}\xspace}          % local estimated variance at point x
\newcommand{\shx}{\ensuremath{\sh(\xv)}\xspace}            % local estimated uncertainty at point x
\newcommand{\sh}{\ensuremath{\hat{s}}\xspace}              % local estimated uncertainty
\newcommand{\px}{\ensuremath{\boldsymbol{x}^*}}
\newcommand{\equote}[1]{``#1''}
\newcommand{\vecx}{\ensuremath{\boldsymbol{x}}}
\newcommand{\yx}{\ensuremath{y(\vecx)}}
\newcommand{\X}{\ensuremath{\mathcal{X}}\xspace}           % domain / search space

% already defined in basic-math:
% \newcommand{\yv}{\boldsymbol{y}}
\newcommand{\fhx}{\ensuremath{\fh(\xv)}\xspace}            % surrogate (x), better use \mhx for predicted value

==> latex-math/ml-trees.tex <==
% ml - trees, extra trees

\newcommand{\Np}{\mathcal{N}}												% (Parent) node N
\newcommand{\Nl}{\Np_1}														% Left node N_1
\newcommand{\Nr}{\Np_2}														% Right node N_2
\newcommand{\pikN}{\hat{\pi}_{\Np k}}             % estimated class probability in N

